A Secure Data Enclave and Analytics Platform for Social Scientists

Data-driven research is increasingly ubiquitous and data itself is a defining asset for researchers, particularly in the computational social sciences and humanities. Entire careers and research communities are built around valuable, proprietary or sensitive datasets. However, many existing computation resources fail to support secure and cost-effective storage of data while also enabling secure and flexible analysis of the data. To address these needs we present CLOUD KOTTA, a cloud-based architecture for the secure management and analysis of social science data. CLOUD KOTTA leverages reliable, secure, and scalable cloud resources to deliver capabilities to users, and removes the need for users to manage complicated infrastructure. CLOUD KOTTA implements automated, cost-aware models for efficiently provisioning tiered storage and automatically scaled compute resources. CLOUD KOTTA has been used in production for several months and currently manages approximately 10TB of data and has been used to process more than 5TB of data with over 75,000 CPU hours. It has been used for a broad variety of text analysis workflows, matrix factorization, and various machine learning algorithms, and more broadly, it supports fast, secure and cost-effective research.

==> background.tex <==
\section{Requirements}
\label{sec:background}
%
%Cloud computing provides a number of capabilities such as elastic capacity and 
%pay-as-you-go usage models, that are particularly attractive to
%scientific users due to the growth of datasets and
%sporadic usage patterns.  
%High resolution acquisition equipment, large sensor networks, 
%and automatically mined datasets are three examples of the 
%trend towards big data science. This, combined with the fact that researchers
%typically aim to analyze as much data as possible as soon as it becomes
%available motivates the need for such cloud platforms. \NAME aims to pass on the advantages of cloud computing models
%to users in a way that simplifies and abstracts the 
%underlying computational infrastructure. 

%Here we briefly describe these use cases and their requirements.

%\textbf{Managing Community Datasets}. 
\NAME is designed to address the requirements
of two canonical use cases: securely managing community datasets and
providing scalable compute resources. There is a growing need for 
researchers to make valuable datasets
available to certain research communities. This might be motivated
by funding agencies or institutions themselves, however, it is generally helpful 
to share data when establishing new research groups. 
%Often, community datasets are valuable, proprietary, or sensitive. 
%They are often created as the result of painstakingly procurement and curation. 
The most important requirements for this use case are that a system be:

\begin{itemize}
	\item Secure: Data should be securely stored and accessible only to
	authorized and authenticated users. 
	\item Scalable: Data can be large, the storage system should scale
	to the data.
	\item Reliable: Data should be stored reliably and available for 
	backup in case of failure or corruption.
	\item Available: Data should be available to 
	geographically distributed users.
	\item High performance: Large amounts of data should be able to be
	moved quickly for analysis, download, and archival.  
	\item Cost-effective: Costs associated with data storage should
	be minimized to encourage use.
	\item Analyzable: The value of data is derived from analysis,
	so it must be easily available for use in compute jobs.
\end{itemize}

%\noindent
%\textbf{Scalable Computing Models}.
Data-intensive research has changed the very basis
of scientific discovery. As data sizes grow and analyses
become more computationally intensive, the requirements often exceed the
computational capabilities of individual researchers. As such, 
researchers need to be able to scale analyses from individual
computers to distributed, parallel modes of computing. To address
these priorities, a system should be:
%Moreover, users accessing community datasets require methods
%with which they can simply analyze data using a variety of
%analysis algorithms. 

\begin{itemize}
	\item Secure: Authorizations should control what data can be analyzed and 
	analyses should be isolated. 
	\item Scalable: Analyses should scale to data, exploit
	parallelism where possible, and leverage large scale computing infrastructure
	for efficient performance. 
	\item Cost-effective: Costs should be comparable or lower than
	using local compute resources.
	\item Easy to use: Interfaces should make it simple to access the 
	underlying infrastructure. 
	\item Colocated with data: Moving data can be costly and slow. 
	Where possible, compute workloads
	should be assigned so they minimize data transfers.
\end{itemize}


==> evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}
Our evaluation explores several important aspects of \NAMENS.
First, we investigate the benefits of elastically
provisioning resources in terms of cost and makespan.
Second, we evaluate the throughput of the system using
a worst-case, many small jobs workload.
Finally, we further explore the potential benefits of
cost-aware provisioning while considering the cost of data transfer. 

%Specifically, the
%
%Three part evaluation :
%\begin{enumerate}
%\item{Evaluate scaling methods from cost vs makespan}
%\item{Evaluate throughput}
%\item{Evaluate strategies for scale of distribution}
%\end{enumerate}

\yadu{Security ? Accesses approved, denied rates so far? Unknown accesses cannot be accounted for}
\yadu{Reliability ? Machines lost, mid run ?}

\subsection{Simulation Workload}

To evaluate \NAME under a realistic usage scenario a simulation
workload was created to mimic existing production
usage of \NAME (see Section~\ref{sec:applications}).
To reduce costs of experimentation, the workload
consists of 40 jobs submitted over a four hour period.
The inter-arrival time is obtained from a Poisson distribution
of the form $t \sim \mathcal{P}(\lambda=0.1667)$ hours.
Where $\lambda$ was selected based on the duration of the experiment.
Within the workload three distinct job types were modeled, representative
of the three distinct analyses that have been executed on \NAMENS.
Specifically, jobs were configured to run for
1, 3, and 4 hours, with 40\%, 20\% and 40\% in each category, respectively.
Each job duration was further varied by up to $\pm5\%$ minutes to
ensure the results are not biased toward hourly increments.
To model data transfer time we randomly assigned input datasets of
$\{1,3,5,7,9\}$ GB. These datasets were hosted on S3. 
%were staged into an instance before execution.
The jobs themselves were comprised of simple calls to \texttt{sleep()}.

\subsection{Elastic Scaling}

\begin{figure}
  \center
  \includegraphics[width=\textwidth]{exp12.png}
  \caption{Elastic scaling in \NAMENS. The top plot shows currently provisioned nodes and the proportion of which are idle. The bottom plot shows each job's status from submission to completion, including wait and data staging time.}
  \label{fig:exp12}
\end{figure}

\NAME embraces on-demand and elastic cloud computing capacity by dynamically provisioning
new instances to host submitted workload.
Note that there is no scheduler, as such, in the sense of a time-sharing system.
Instead, scaling is achieved by provisioning instances as the need arises based on the state of the queue.
%Two experiments on simulated workloads and two the results on two production use-cases are reviewed.
For each experiment we compared the trade-offs between total execution time (``makespan'') and total cost.
%In each case, time and cost are analyzed with respect to the mixture of time in various stages and the location of data.
%A key component to \textsc{Kotta Cloud} is its tiered storage strategy, which has an effect on latency when staging-in data.
%The data layer is also affected by \textit{where} the data is stored geographically.
%The evaluations show that the location of the data is crucial to minimizing cost, even at the expense of node-provisioning cost.
Three scaling strategies were explored:
\begin{itemize}
    \item \textbf{No scaling}: A baseline strategy in which a fixed number of instances are provisioned.
    \item \textbf{Limited scaling}: A restricted strategy where the maximum number of provisioned nodes is limited.
%	This configuration models a restriction placed on the system by administrators with the goal of reducing costs.
    \item \textbf{Unlimited scaling}: An unbound strategy where as many instances as are needed will be provisioned. 
\end{itemize}

%\subsubsection{Strategy 1: No scaling}
%This experiment uses a fixed number of instances that are provisioned ahead of time. We evaluate the makespan and the total compute costs incurred as we use a series of jobs arriving in Poisson distribution over
%the span of 4 hours. This is the benchmark against which we will compare the remaining strategies.
%
%\subsubsection{Strategy 1: Unlimited Scaling}
%The goal of the first experiment is to demonstrate that automatic scaling performs well for workloads randomized in various ways. To demonstrate the functional and cost advantages, tasks loads were designed to simulate expected workload patterns. These include medium--duration jobs ranging from 1 to 4 hours. To simulate the expected workload 40 jobs were submitted over four hours arriving at intervals sampled from limited Poisson distribution of the form $t \sim \mathcal{P}(\lambda=0.1667)$ hours each. The duration of each task is also varied by $\pm5\%$ minutes. The tasks themselves consist of calls to \texttt{sleep()} after staging-in a file of size $\{1,3,5,7,9\}$ GB.
%
%\subsubsection{Strategy 2: Limited scaling}
%Here, we consider the cases where provisionable resources are restricted to 10 and 20 nodes each.
%The evaluation simulates circumstances where administrators may attempt to minimize costs by restricting
%the provisionable number of nodes. While this it ostensibly a reasonable strategy, as we will see,
%\NAMENS's provisioning sub-system is able to provision and tear down nodes quickly enough that
%the result is longer wait-times with negligible cost savings.

\figurename~\ref{fig:exp12} illustrates the relationship between job execution
and the elastic infrastructure provisioned to host the workload when using the unlimited
scaling strategy.
% the lifecycle of every job in the workload using the
%unlimited scaling strategy.
For each job, it shows
the time of submission, the wait time in a queue before execution began,
the data staging time (in/out), and the execution time.
%% I feel like the caption says all this, and we've already pointed people to it: // AG
%The top figure shows the number of cloud instances provisioned to host the workload, it
%also shows the number of provisioned instances that are idle at any point in time.
The results highlight \NAMENS's ability to elastically provision infrastructure
for waiting jobs. The workload peaks at 27 concurrent jobs.
The results also show a moderate wait time due to the delay caused by
provisioning instances, which, on average is 7:39 per job with a 
peak of 30 minutes due to spot market volatility.
The advantage of reusing existing instances is evident in the figure:
the last 7 jobs were able to execute without waiting because idle instances were
available in the pool.

Table~\ref{table:provisioning} compares the different scaling strategies with respect
to makespan, cost, and wait time.
Wait time is the time a job waited in the queue.
Makespan records the total execution time from when the first job is first submitted until the last
job completes.
Spot costs were calculated as the cost paid for running the experiment
using Spot instances.
Note that these experiments were run at different times with
different market conditions, therefore the spot costs may vary significantly
between executions.
The on-demand cost was calculated based on the price that would have been
paid had on-demand instances been used. These
results aim to remove the variability of the spot market when comparing costs.
The cost savings, then, are the percentage improvement
compared to the baseline (no scaling, min: 40, max: 40) strategy.

The no scaling strategy, where a fixed pool of instances are available to host
the workload, represents a baseline strategy to which the others can
be compared. Using a fixed pool of 40 instances, the wait time is 0, optimizing
the makespan. However, many instances are idle for a significant portion
of the workload which results in costs of \$74.57 for 40 fixed instances
and \$40.87 for 20 fixed instances.
The unlimited scaling strategy provisions instances only when they are required.
Here the wait time is longer than the no scaling strategy (on average 7:39
per job), however the cost of executing the whole workload is significantly lower
(saving approximately 61\% using spot or on-demand instances).
The unlimited scaling strategy using Spot instances offers similar compute performance 
at 1/16th the cost of a static cluster provisioned with on-demand instances.
Note: the makespan is the same as the last jobs to complete do not have to 
wait in the queue as their are idle instances available for execution.
The limited scaling strategies aim to provide a hybrid model to manage
the trade-off between cost and time. As expected, the results show
increased makespan (roughly 1 hour and 5 hours longer for 20 and 10 instances, respectively)
with reduced cost (roughly \$2 and \$5 for 20 and 10 instances, respectively).
Thus, when administrators have knowledge of potential workloads, they can define 
scaling restrictions to minimize idle times
and reduce costs.

%\todo[inline]{1p results on time, cost \& overhead and a conclusion that limits are more costly than helpful.}
\bgroup
\def\arraystretch{1.2} % Cell padding
\begin{table*}
  \centering
  \label{table:provisioning}
  \caption{Cost vs. Makespan.}
  {\footnotesize
    \begin{tabular}{lllllcccc}
    \hline
    \input tables/cost_makespan.tex
    \hline
    \end{tabular}
  }
\end{table*}
\egroup

\subsection{Throughput}
To evaluate the throughput of \NAME we designed a strong scaling experiment where 10,000
small tasks were submitted to a pool of general purpose instances (m4.xlarge, 4 cores@2.4Ghz).
To model a worst-case scenario, each task is a \texttt{sleep(0)} call and requires
no data staging.
Instances were provisioned ahead of time to reduce overhead associated with the provisioning process.
We measure the total time to completion of the 10K tasks for $\{1,2,4,8,16,32\}$ worker nodes.
In an ideal case, we should observe speed-ups directly proportional to the number of nodes.

\begin{figure}
  \center
  \includegraphics[width=0.475\textwidth]{tput_test.png}
  \caption{Throughput in \NAME for 10,000 tasks}
  \label{fig:throughput}
\end{figure}

\figurename~\ref{fig:throughput} shows the time to submit all 10,000 tasks, the total time to completion
for tasks on provisioned instances, and the throughput.
The results show that throughput increases linearly with the number of worker nodes
up to 16 nodes. Up to this point, the average task throughput per worker node is 4.90 tasks/s (total 79.84 tasks/s).
The primary bottleneck in this experiment is the database as transactions are used to record job descriptions and
performance markers. For these experiments we increased the DynamoDB read and write capacity per second to 100 and 400, respectively.
It is important to note that these experiments represent an idealized worst case
scenario where tasks are trivial. With more typical, longer running jobs on the order of
minutes or hours, the results show that \NAME can easily support thousands
of jobs submitted simultaneously.

\subsection{Cost-aware Provisioning}

\NAME uses Spot instances to reduce costs.
Here we explore the benefits of various strategies in the context of geographically distributed computation in a cloud environment.
In this experiment data was hosted in one region (N.Virginia, us-east-1) and compute was distributed across different EC2 regions and AZs.
We use historical spot price data from ten AZs spread across four regions, and simulate various strategies for instance selection.
We simulate a single hour task that is provisioned among the AZs based on the different strategies.
This simulation is executed for a month to capture the long term impact of price differences between AZs.

We calculate the total cost of computation for a given hour $P_{total}$,
as the sum of the hourly instance price $P_{i}$ and the costs
associated with data transfer.
\begin{equation}
\label{eqn:1}
    P_{total} = P_i + P_{transfer}
\end{equation}
If the selected compute instance lies in a different region than the location of the
S3 data bucket, there is an inter-region data transfer cost $T_{c} = \$0.020/GB$ ~\cite{s3_transfer_cost}.
The amount of data downloaded and uploaded from S3 are represented by $D_{dn}$ and $D_{up}$, respectively,
which we assume to be equal.
%The simulation considers varying data volumes and its impact on cost.

\begin{equation}
\label{eqn:2}
 P_{transfer} =
\begin{cases}
    0 ,& \text{if } us-east-1\\
    (D_{dn} + D_{up}) \cdot T_c, & \text{otherwise}
\end{cases}
\end{equation}

\begin{figure}
  \center
  \includegraphics[width=0.475\textwidth]{c4_8xlarge_pricing_simple.png}
  \caption{Monthly cost for C4.8xlarge instance with data egress costs.}
  \label{fig:cost_data_egress}
\end{figure}

%\kyle{Why is this cost per month? What is the workload?}
%\yadu{I simulated a workload over a month which consisted of 1 hour tasks for the entire duration, and switched instances every hour among the AZ's.}

\figurename~\ref{fig:cost_data_egress} shows the total monthly cost of using C4.8xlarge
instances when different amounts of data are used by the analysis. 
The graph shows several different provisioning strategies: 
selecting the cheapest or most expensive instance in a single AZ,
the cheapest instance across AZs, and the cheapest instance across regions.
The graph also shows the savings that are obtainable when broadening 
the search scope across AZs and regions.
The results show a significant difference between the cheapest and most expensive
instance within an AZ. This suggests there is considerable financial risk when provisioning
instances within a single AZ.  Thus, there is considerable advantage to 
selecting instances across AZs and regions. However, we observe diminishing returns from 
extending the search scope to consider multiple regions
as the volume of data transfer associated with compute tasks increase.
This result confirms the need to co-locate compute with data as data sizes increase.

